Optimally Leveraging Density and Locality to Support LIMIT Queries

Existing database systems are not optimized for queries with a LIMIT clause---operating instead in an all-or-nothing manner. In this paper, we propose a fast LIMIT query evaluation engine, called NeedleTail, aimed at letting analysts browse a small sample of the query results on large datasets as quickly as possible, independent of the overall size of the result set. NeedleTail introduces density maps, a lightweight in-memory indexing structure, and a set of efficient algorithms (with desirable theoretical guarantees) to quickly locate promising blocks, trading off locality and density. In settings where the samples are used to compute aggregates, we extend techniques from survey sampling to mitigate the bias in our samples. Our experimental results demonstrate that NeedleTail returns results 4x faster on HDDs and 9x faster on SSDs on average, while occupying up to 23x less memory than existing techniques.

==> generalization.tex <==
%!TEX root=main.tex


\section{Generalizations}
\label{sec:extensions}
So far, we have assumed that all our sampling queries have the form
dictated by the SELECT query given in Section~\ref{sec:prob}, thus limiting our
operations to
a single database table, with simple selection predicates
and no group-by operators.
We now extend the \anyk sampling problem formulation and our
algorithms to handle more complex queries, 
which contain group-by and join operations.

Recall that our \anyk algorithms operate primarily by estimating the densities
of blocks which satisfy the query constraints and choosing a set of blocks based on
their densities and locations.
Our solutions for supporting the group-by and join operations work 
by adapting the notion of density to these operations.
%If we could derive a similar notion of density within the context of blocks from
%group-by and join operations,
%Our solutions for group-by and joins augment the notion of a density 
%The densities in this context represent the
%``usefulness'' of these blocks; blocks which have more valid records are more
%useful since fewer blocks to need be retrieved overall.
%If we can calculate a similar metric of usefulness for blocks in group-by and
%join operations,
By doing so, we can run the same \anyk algorithms introduced in 
Section~\ref{sec:alg} with little modification
for more complex queries.
%In the remainder of this \liqi{appendix}, we outline how we can calculate the
%densities for group-by and join operations.
%\techreport{
%Furthermore, we show that with
%these extensions, \anyk sampling can be applied to the real-world use case of
%quickly generating aggregated visualizations.
%}
%\papertext{We omit many details that can be found in our extended
%technical report~\cite{needletail-tr}.}

%
%In this section, we first describe how we can apply \anyk sampling on join and
%group-by operations. Recall that \thresh and \prong calculate density estimates
%of the query results for each of the blocks to decide which blocks to fetch for
%getting the desired number of samples quickly. For instance, for a conjunction
%selection operation, the density estimates are calculated as the product of the
%densities of attribute values in selection predicates . Here, we outline how we
%can estimate densities of the blocks for group-by and join operations.

\subsection{Supporting Group-Bys}
In \anyk queries we have studied so far, the densities of blocks represent the
\emph{priorities} with which those blocks should be retrieved; denser blocks have
higher priority since they lead to lower I/O times. This idea extends naturally to group-by 
queries, where the goal is produce $k$ samples per group.
The simplest approach is to apply our \anyk algorithms separately on each group in the
group-by operation, creating an extra constraint for each group.
However,
to achieve even lower runtimes, we can augment our notion of priority
to consider every group in a group-by operation, and run the \anyk
algorithm for all groups. 
Our augmented notion of priority for a block should depend on the number of
samples already retrieved for each group and only count valid records
belonging to groups which do not yet have $k$ retrieved samples.

%
%depend on whether groups
%have already retrieved
%$k$ samples and only count the valid records in the block for groups which do
%not yet have $k$ retrieved records.
%
%be based on the number
%
%should assign priorities to blocks
%
%
%With this augmented notion of priority, if a block contains
%valid
%records belonging to different groups, the priority of that block
%should be the sum total number of valid records belonging to groups which
%do not yet have $k$ retrieved samples.
%

More formally, we consider group-by \anyk queries of the form:

\begin{align*}
  &\text{SELECT } \text{\bf ANY-K}(*) \text{ FROM }T \text{ WHERE } S \text{ GROUP BY } A_G
\end{align*}
%where $S$ is the constraints of the query and $A_G$ is the group-by attribute
%consider the priority of a block across
%all groups in the group-by operation, since a given block may contain tuples belonging
%to multiple groups. Initially, when no samples have
%been taken, the priority of a group-by block is simply the sum of the densities of
%the groups within that block. As more samples of a group $G$ have been
%retrieved, there is less need to collect blocks which have a large
%number of group $G$ records. Therefore, to approximate the priorities of
%blocks based on their group proportions, we weigh the densities of groups in
%blocks by the number of samples still needed for that group.
%\papertext{
%  This extension also generalizes to multiple group-by predicates.
%}
%
%%\srm{I think the following math could be cut.  Could say that these ideas generalize to multiple group by predicates without giving the math.}
%\techreport{
%Formally, we let group-by \anyk queries have the form:
%\begin{align*}
%  &\text{SELECT } \text{\bf ANY-K}(*) \text{ FROM }T \text{ WHERE } S \text{ GROUP BY } A_G
%\end{align*}
where $S$ is the query predicate(s) and $A_G$ is the group-by attribute with
$\delta_G$ number of distinct values/groups: $\{V_G^1, V_G^2, ...,
V_G^{\delta_G}\}$.
We can construct two \densitymaps: 1) $D_P$,
which estimates densities of blocks with respect to the predicate $S$, and 2)
$D_G^j$, which estimates the densities of blocks with respect to the group-by value
$V_G^j$, for every group in $A_G$. Using the notation of
Section~\ref{sec:idx} to denote a \densitymap $D_P$ as an array
of densities: $\{d_{P_1}, d_{P_2}, ..., d_{P_{\lambda}}\}$, where
$d_{P_l}$ refers to the density of the $l$th block with respect to $S$,
we can  express our augmented notion of priority as:
\[
  d_{(S, G)_{l}} = d_{P_l} \sum_{j=1}^{\delta_G} w_l(V_G^j)
\]
where $w_l(V_G^j)$ is some heuristic function to represent the weighted density
of the $l$th block
for each group $V_G^j$. As mentioned earlier, one heuristic for $w(V_G^j)$ may
depend on the number of samples already retrieved for $V_G^j$:
\begin{equation}
  w_l(V_G^j) = min\left(k - r_G^j \;, \;d_{G_l}^j \times
  records\_per\_block\right)
  \label{eq:gby-opt-heuristic}
\end{equation}
where $r_G^j$ is the number of samples already retrieved for group $V_G^j$ and
$d_{G_l}^j$ is the density of the $l$th block for $V_G^j$. This heuristic
measures the number of expected valid records in block $l$ for $V_G^j$, but limits
it by the number of samples left to be retrieved for group $V_G^j$. This allows
the valid records belonging to group $V_G^j$ contribute to the overall priority
of the block, but reduces the amount of contribution as more samples of that group have been
sampled. Once all $k$ samples have been retrieved for a group, the valid
records belonging to that group then no longer contribute to the overall priority.

\ntail uses a slightly more advanced heuristic which also includes the inverse
frequency of each group. The intuition is that frequently occurring groups
will appear commonly as a byproduct of retrieving almost any block, so they
should be weighted less in the overall priority, while rarer groups should have
higher priority. Formally, the $w_l$ function used by \ntail is given by:
\begin{equation}
  w_l(V_G^j) = \frac{1}{f_G^j}min\left(k - r_G^j \;, \;d_{G_l}^j \times
  records\_per\_block\right)
  \label{eq:gby-ntail-heuristic}
\end{equation}
where $f_G^j$ is the frequency of group value $V_G^j$ across the entire dataset
and can be estimated as the average density across all blocks:
\[
  f_G^j = \frac{1}{\lambda} \sum_{l=1}^{\lambda} d_{G_l}^j
\]

With the augmented notion of priority, we can now construct an iterative
\anyk algorithm for group-by operations, similar to the algorithms in
Section~\ref{sec:alg}. The main structure of the algorithm is as follows:
\begin{inparaenum}[(1)]
\item
  Update all densities  using $w_l$.
\item
  Run one of the \anyk algorithms to retrieve $\psi$ blocks with the highest
  priority (which have not been retrieved yet).
\item
  If $k$ samples still have not been retrieved for each group, go back to step (1).
\end{inparaenum}
Since our augmented notion of density depends on the number of samples already
retrieved, the densities must be updated periodically to ensure the correctness
of the priorities. The $\psi$ parameter controls the periodicity of these
updates. The problem of setting $\psi$ becomes a trade-off between CPU time and
I/O time.
Setting $\psi=1$ updates the densities after every block retrieval; while this
more correctly prioritizes blocks and is likely to lead to fewer blocks
retrieved overall, there is a high CPU cost in updating the densities after each
block retrieval. As $\psi$ increases, the CPU cost goes down due to less frequent
updates, but the overall I/O cost is likely to go up since the priorities are
not completely up-to-date for each block retrieved.

The full algorithm for the group-by \anyk query is shown in
Algorithm~\ref{alg:group-by}. In Section~\ref{sec:alg}, $\tau$ was a single
value representing the number of samples retrieved; for the group-by \anyk
algorithm, $\tau$ is now an array of size $\delta_G$ where each entry
represents the number of samples for that group.
Every iteration
consists of updating the priorities of blocks $M$ based on the number of samples
retrieved (setting it to 0 if it has already been seen), and calling an \anyk
algorithm with $M$ and the number of blocks desired back $\psi$. The algorithm
updates the counts of $\tau$ and the algorithm only ends once every entry in
$\tau$ is at least $k$.

{\small
\begin{algorithm}
\caption{Group-by \anyk algorithm.}\label{alg:group-by}
\begin{algorithmic}[1]
  \State Initialize $\tau \gets [0,...,0]$, $R, M \gets \varnothing$

\While{$\exists j \in \{1,...,\delta_G\}, \; \tau[j] < k$}
\For {$i = 1 \dots \lambda$}
\If{$i \in R$}
\State $M[i] \gets \left\{
  \begin{array}{ll}
    bid: & i \\
    density: & 0 
  \end{array}
  \right.$
  \Else
  \State $M[i] \gets \left\{
  \begin{array}{ll}
    bid: & i \\
    density: & d_{P_l} \sum_{j=1}^{\delta_G} w_l(V_G^j)
  \end{array}
  \right.$
  \EndIf
  \EndFor
  \State $R' \gets \text{\anyk}(M, \psi)$
  \For{$r \in R'$}
  \For{$j \in \{1,...,\delta_G\}$}
  \State $\tau[j] \gets \tau[j] + d_{P_r} d_{G_j}^r \times records\_per\_block$
  \EndFor
  \EndFor
  \State $R \gets R \cup R'$
\EndWhile
\State \textbf{return} $R$
\end{algorithmic}
\end{algorithm}
}

\stitle{Optimal Solution}
As mentioned, the group-by solution used by \ntail uses a heuristic to find the
best blocks to retrieve. However, an I/O optimal solution, similar to \optimal from
Section~\ref{subsec:optimal}, could be derived using dynamic programming with 
a recursive relationship based on the notion of priority from
Equation~\ref{eq:gby-opt-heuristic}, $\tau$, and the disk model from
Section~\ref{subsec:optimal}. Unfortunately, the resulting dynamic programming
solution becomes a complex program of even more dimensions
than the program from Section~\ref{subsec:optimal}. Since we
already showed in Section~\ref{sec:eval} that \optimal incurs a prohibitively
high CPU cost in exchange for its optimal I/O time, we chose not to pursue this
avenue.

\stitle{Multiple Group-Bys} For multiple group-by attributes, we simply extend
the above formula to account for every possible combination of values from the
different groupings. For example, if we have two group-by attributes $A_G$ and
$A_{G'}$ with \densitymaps $\{D_G^1, ..., D_G^{\delta_G}\}$ and $\{D_{G'}^1,
  ..., D_{G'}^{\delta_{G'}}\}$ respectively, we can specify our updated notion
  of density with:
\[
  d_{(P, G, G')_{l}} = d_{P_l} \sum_{j=1}^{\delta_G}
  \sum_{i=1}^{\delta_{G'}} w_l(V_G^j) w_l(V_{G'}^i)
\]


\subsection{Supporting Joins}
\ntail supports natural foreign key/primary key joins. We define \anyk sampling
for joins as retrieving $k$ samples for each distinct join value. For example,
if we want to join on a ``{departments}'' attribute, $k$ samples would be
retrieved for each department. With this definition, the problem of supporting
joins can be reduced to the exact same problem as supporting group-bys. Each
join value becomes a group value from the previous section, and
Algorithm~\ref{alg:group-by} can be used to find the best blocks for a join
operation. More formally, we assume an \anyk join query has the form:
\begin{align*}
  &\text{SELECT } \text{\bf ANY-K}(*) \text{ FROM }T \text{ JOIN }T' \text{ ON }
  T.A_J = T'.A_J
\end{align*}
where $T'$ is the table in which the join attribute $A_J$ is the primary key and
$T$ is the table in which $A_J$ is the primary key. \ntail first scans $T'$ to
gather all possible join values, then runs the group-by \anyk algorithm on table
$T$ with $A_J$ as the group-by attribute:
\begin{align*}
  &\text{SELECT } \text{\bf ANY-K}(*) \text{ FROM }T \text{ GROUP BY } A_J
\end{align*}
The resulting blocks indicate the best blocks that \ntail can retrieve to
minimize the overall time for \anyk sampling for joins.
%\stitle{Join}
%%\srm{I don't understand the goal?  Is it to produce a sample of k records for each distinct join value?  What if there are fewer
%%than k matching values for a given value?  }
%Our goal for \anyk sampling for the natural join operation is retrieve \anyk
%samples from the space of all joined valid records.
%%Similar to group-bys, our goal for a natural join
%%operation is to retrieve \anyk samples for each value joined upon.
%Typically,
%the natural join operation between table $T$ and table $T'$ on attribute $A_J$ requires
%a cross product between all blocks in $T$ and $T'$ to match the values of
%$A_J$. However, an advantage of \anyk sampling is that we can avoid doing the
%full cross product because we only need $k$ results. The core idea
%%in extending
%%our \anyk algorithms for join operations
%is to retrieve the densest blocks for
%both tables $T$ and $T'$ and perform a smaller cross product among these blocks
%to retrieve as few blocks as possible.
%\techreport{
%More formally, we assume that a join query has the form:
%\begin{align*}
%  &\text{SELECT } \text{\bf ANY-K}(*) \text{ FROM }T \text{ NATURAL JOIN }T' \text{ WHERE } P \text{
%  AND } P'
%\end{align*}
%where $P$ are the predicates pertaining to table $T$, $P'$ are the
%predicates pertaining to table $T'$, and $A_J$ with values $\{V_J^1, V_J^2,
%..., V_J^{\delta_J}\}$ is the attribute that is being joined on.
%
%Given these assumptions, we first perform the group-by \anyk algorithm with
%\densitymaps $D_P$ and $D_J^j$ for every $j \in \{1, ..., \delta_J\}$ (i.e., we treat $A_J$ as
%the group-by attribute) for table $T$, and we call the resulting set of
%blocks $B_T$. Then we similarly perform the group-by \anyk algorithm with
%\densitymaps $D_{P'}$ and $D_J^j$ for every $j \in \{1, ..., \delta_J\}$ for
%table $T'$ and call the resulting set of blocks $B_{T'}$. For every pair of
%blocks $\{(b, b') \; | \; b \in B_T, b' \in B_{T'}\}$, we calculate the
%priority for that block pair with:
%\[
%  d_{b,b'} = d_{P_b} d_{P'_{b'}}\sum_{j=1}^{\delta_J} w_J^j d_{J_b}^j d_{J_{b'}}^j
%\]
%where $w_J^j$ is the once again the weight introduced based on the number of
%samples needed for join value $V_J^j$. We can retrieve the blocks based on
%these calculated priorities to minimize the total I/O time. If not enough
%records were retrieved from the first cross product, or if the number of
%samples retrieved for different join values is greatly skewed, we 
%reiterate the entire process again.
%}
We leave optimizations for other join variants for future work.

%Unlike selection and group by operations, for join operation we
%need to find the best combinations of blocks from different tables involved in
%join that minimize the overall random IO. For natural join the density
%estimates for a combination of blocks (one block from each table) can be the
%weighted sum of the product of the densities of the blocks for each of the
%distinct values of the join attribute. For instance, if we have a natural join
%on an attributes $A_i$ across two table T1 and T2, the density estimate for
%block $x$ in T1 and block $y$ in T2 is equal to $\sum_{j=1}^{\delta_i}
%(w_{i1}^j.w_{i2}^j.d_{ij}^x.d_{ij}^y) =w_{i1}^1.w_{i2}^1.d_{i1}^x.d_{i1}^y +
%w_{i1}^2.w_{i2}^2.d_{i2}^x.d_{i2}^y + ... +
%w_{i1}^{\delta_i}.w_{i2}^{\delta_i}d_{i\delta_i}^xd_{i\delta_i}^y$ where
%$w_{i1}^j=\frac{n_i^j}{\sum_{j}n_i^j}$ in Table 1. \silu{What is the rational
%of using $w_{i1}^j$ here? Do we want to ensure that in the join results, the
%number of tuples are proportional to $n_i^j$ as in Group By query?} To do this
%efficiently using Algorithm \ref{alg:threshold}, we first create sorted Density
%Maps for each attribute value, each entry in the Density Map corresponds to a
%combination of blocks from different tables stroing the product of their
%densities. Then, using \thresh we pick a few blocks with the highest densities
%to collect k samples. In a similar fashion, we can apply \anyk sampling on
%other types of join by modifying the density estimates.

\subsection{\Anyk Sampling for Visualizations}
%\textbf{\Anyk Sampling for Visualizations}:
Many data analysts derive insights from aggregate visualizations such as line
charts, histograms, and bar charts. However, when the datasets are too large,
the time taken to generate these visualizations are too long to be considered
interactive. Most aggregate-based visualizations retrieve data using the
following format:
\[
  \text{SELECT } X, Aggr(Y) \text{ FROM } T \text{ WHERE } P \text{ GROUP BY }
  X
\]
where $Aggr(Y)$ is some aggregate of $Y$ such as $AVG(Y)$ or $SUM(Y)$. For
these types of queries, we can use aggregate estimators from
Section~\ref{sec:est} in addition to the group-by extensions from this section
to minimize the data retrieval time for these visualizations.

%\textbf{Any-k sampling for generating fast aggregated visualizations}:  Data
%analysts mostly derive insights through interactive exploration of their
%datasets using aggregate visualizations such as line charts, histograms, bar
%charts. However, when the datasets are large, these visualizations take a large
%amount of time to be generated. Approximate visualization systems based on
%random sampling techniques work well when the data is stored in memory, but
%incur high latency when the data is stored in disk - mainly due to random disk
%IOs. Any-k samples in combination with a much smaller number of random samples
%can result in a massive speed up of the response time with a similar or marginal
%decrease in accuracy.  

Similarly, \ntail can be used as a sampling engine  for various analytical and
statistical tasks used in decision support systems that demand increasingly
faster
response times. Currently, most of these tasks do not scale to the hundreds of
terabytes of data often found in modern data warehouses, and \ntail can help in
making these tasks more interactive.
%\tar{need to extend it further} \silu{Do we
%want to claim that \ntail can be used in sampling engine? The concern is that
%this may attract reviewers' attention and they may criticize it on lacking of
%theoretical guarantee.}


==> theory.tex <==
\section{Analysis of Sampling}
Have analysis here which shows taking any-k of large amounts of records gives
us some sampling guarantees.

